CitySurfaces: City-Scale Semantic Segmentation of Sidewalk Materials

While designing sustainable and resilient urban built environment is increasingly promoted around the world, significant data gaps have made research on pressing sustainability issues challenging to carry out. Pavements are known to have strong economic and environmental impacts; however, most cities lack a spatial catalog of their surfaces due to the cost-prohibitive and time-consuming nature of data collection. Recent advancements in computer vision, together with the availability of street-level images, provide new opportunities for cities to extract large-scale built environment data with lower implementation costs and higher accuracy. In this paper, we propose CitySurfaces, an active learning-based framework that leverages computer vision techniques for classifying sidewalk materials using widely available street-level images. We trained the framework on images from New York City and Boston and the evaluation results show a 90.5% mIoU score. Furthermore, we evaluated the framework using images from six different cities, demonstrating that it can be applied to regions with distinct urban fabrics, even outside the domain of the training data. CitySurfaces can provide researchers and city agencies with a low-cost, accurate, and extensible method to collect sidewalk material data which plays a critical role in addressing major sustainability issues, including climate change and surface water management.

==> old/conclusion.tex <==
\section{Conclusion}
We present CitySurfaces, a scalable, low-cost approach towards the automatic computation of the spatial distribution of pavement materials at the sidewalk segment level. Our model can detect a diverse range of materials, which to our knowledge, were not covered by any existing dataset.
%
For instance, hexagonal pavers or granite blocks were not reported in any sidewalk inventories reviewed in this study. CitySurfaces produces accurate segmentation acquired from multiple cities both within and outside the domain of the training data, demonstrating generalization capabilities across varying urban fabrics. 
%
CitySurfaces can detect, delineate, and classify eight  standard surface materials used throughout most US cities. As shown in Section~\ref{block(c)}, the framework can be extended to include additional surface materials with less effort than building a city-specific model from scratch, which makes it possible for almost any city or government agency that has spatially dense street-level image data, to create a similar dataset.
%
Moreover, since we have covered the standard materials, such as concrete, asphalt, granite / bluestone, and brick, our model can be applied to a wide range of cities without any further annotation effort or with substantially less effort using our pre-trained model. \highlight{We will make our models as well as the datasets generated for the six selected cities publicly available through a GitHub repository. }

This work has addressed some challenges in data annotation and accurate classification of different materials with high between-class similarities and within-class variation. The active learning framework utilized in this study helped reduce the annotation costs by choosing the most informative set of data to be annotated and incrementally decreasing the manual modification time. 
%
By offering the first comprehensive dataset of sidewalk surface materials at the city scale, this study goes beyond reporting the dominant material of each segment and provides information on the percentage distribution of all detected materials per sidewalk segment. \removed{which combined with external data such as fine-scale shadow accumulation~\citep{shadowmap} can provide a more precise city-wide estimation of the surface UHI.} \highlight{Our material classes in this study were selected based on the standard surface materials listed by Boston sidewalk inventory~\citep{Bostonswinv}, to use it as our baseline ground truth. That list, is not extensive and does not distinguish between various types of the same class of material such as concrete. However, for some more in-depth analysis, such as measuring UHI, we may need to classify the materials differently, and distinguish between different variation of the same material within one class. For instance, reflective granite and dark matte bluestone should have two distinct classes, same goes with the dark and light concretes since they have distinctively different albedo values. CitySurfaces framework can be easily extended to detect more classes of materials as illustrated with the Manhattan example explained in Section~\ref{block(c)}, given the availability of the images corresponding to each class of interest to create the initial ground-truth set. In our future work, we plan to take these consideration into account and combine our generated data with shadow accumulation~\citep{shadowmap} to generate a city-scale UHI map.}

To facilitate designing automated audit tools, we are going to extend our model to detect surface problems such as potholes, significant breakage, and obstacles on pedestrian paths for accessibility analysis. We also aim to address the walkability and active design of sidewalks by developing a model to detect the relevant features of the sidewalks wall plane and furnishing zone, such as window-to-wall ratio.
%
As another line for our future work, we would like to explore automated sample selection procedures and self-supervised learning techniques and tailor them to sidewalk and pedestrian facility analysis. 
%
We chose a simple (yet effective) uncertainty measure and coupled it with the analysis of the model's performance on the validation set and used expert's feedback to refine our annotations and to check whether the model is predicting correctly since, on many instances, it is difficult to distinguish between visually similar materials. 


==> old/data.tex <==
\section{Data Description} 
\label{data}

\subsection{Boston Sidewalk Inventory}
\label{data:boston} 

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figs/materials_compressed.pdf}
\caption{\removed{The eight classes of surface materials used in our study. The top row presents standard and prevalent materials found in most of the cities. The
mixed class is the next popular one and the three remaining materials in the second row have distinct use. Cobblestone is street pavement material, mostly
seen in historic neighborhoods.} \highlight{The eight classes of surface materials used in our study. Top: standard and prevalent materials, Bottom: Materials with distinct use}}
\label{fig:materials}
\end{figure}

The sidewalk inventory~\citep{Bostonswinv} is part of the Boston~Pedestrian~Transportation~Plan~\citep{bostonregional} and describes sidewalk features, including geographic coordinates and paving materials collected via manual field visits. The material attribute describes the dominant surface material of each street segment (either concrete, brick, granite, a mix of concrete and brick, or asphalt). Fig.~\ref{fig:materials} illustrates patches of these five materials; the other three extra materials (granite block, cobblestone, hexagonal pavers) shown in the image were not recorded in the Boston dataset but were later manually added to our classes, as we will discuss in Section~\ref{block(c)}. We grouped the street segments by materials, using the geographic coordinates of the paving materials in the Boston inventory,  and used it to assign an overall image class to the street-level images to guide the annotation process. 


% The distribution of surface materials varies strongly across Boston. Concrete and mix of concrete and bricks were the most prevalent materials, with brick and asphalt coming second and granite sidewalks being the rarest, as shown in Fig.~\ref{fig:radardiagram}. 


\subsection{Street-level Images}
\label{data:gsv}

Street-level image usage in urban analysis has gained popularity with the introduction of Google Street View (GSV)~\citep{anguelov2010google} and Microsoft Street Slide~\citep{kopf2010street}, services that provide panoramic images captured by specifically designed cameras mounted on a fleet of vehicles. These new data sources enable new questions and study designs for urban planning and design, urban sociology, and public health~\citep{griew2013developing,yin2015big,mooney2016use}.  The GSV API can retrieve street-level images via geographic coordinates and allows users to adjust camera settings such as the heading, field of view (FoV), and pitch.

\begin{figure}[h!]
\centering
\includegraphics[width=0.5\textwidth]{figs/segmentation-1.pdf}
\caption{Examples of sampled points in Boston to obtain street-level images. Three different sampling locations are highlighted and for each location, the street-level image as well as the prediction result of the model is depicted.}
\label{fig:gsv-diverse}
\end{figure}


We use the OSMnx library~\citep{boeing2017osmnx} to obtain the Boston street network and query the GSV API for street-level images at a fixed interval~(5 meters), excluding major highways and tunnels. We acquire the compass bearing of each street to set the camera heading to be perpendicular to the street, thus looking directly at left and right sidewalks. The pitch was set to $0^{\circ}$ with an FoV of $80^{\circ}$. To create a more diverse training set, for 35\% of the training data, we use different combinations of headings (pitch $\in[-10^{\circ}, -20^{\circ}$], and FoV$\in [60^{\circ}, 70^{\circ}$]), to have sidewalk images taken at varying angles and perspectives. Fig.~\ref{fig:gsv-diverse} illustrates sampled street segments in Boston, together with their image-level annotations. In order to train our framework, 3,500 Boston images were obtained, and later 2,000 images from NYC were added to our pool of initially unannotated data. We excluded images with no sidewalks as well as those where more than 80\% of the sidewalks were occluded. The final set had a total of 4,300 images.



==> old/discussion.tex <==
\section{Discussion}
\label{discussion} 

\begin{figure*}[t!]
\centering
\includegraphics[width=0.8\textwidth]{figs/failures_compressed.pdf}
\caption{\removed{Objects with patterns similar to different materials. Left: Random patterns created by different objects led to misclassifications. Left top: Plant pit
was classified as brick, and then model predicted mixed class instead of concrete for that part of sidewalk segment. Left middle: Broken parts of concrete
were classified as small stones. Left bottom: The brownish metal covers were classified as brick, leading to the perdition of mixed class instead of concrete.
Right: using an active learning approach, the model corrects itself and, in the final cycle, predicted correct classes in similar settings.}~\highlight{Objects with patterns similar to different materials. \textbf{Left}: Random patterns created by different objects led to misclassifications. \textbf{Left top}: Concrete alongside a furnishing zone was misclassified as mixed class since plant pit was detected as bricks, ~\textbf{Left middle}: Broken concretes were misclassified as granite blocks, \textbf{Left bottom}: Concrete was misclassified as mixed class due to the presence of brownish metal covers. \textbf{Right}: The results of the final cycle with active learning approach and correct predictions in similar settings.}}
\label{fig:failures_material}
\end{figure*}

%
The specific characteristics of computing the spatial distribution of sidewalk pavement materials require experts to oversee the performance of the model and ensure that the network is correctly classifying the pavement materials. 
%
Through our active learning process, we identified certain elements of the urban scenes that can create higher prediction confusion and lead to misclassification. 
%
Two main categories of patterns that were repeatedly observed among the failure cases were shadow/light contrasts (Fig.~\ref{fig:failures_light}) and distinct objects such as metal gratings and plant pits that resemble brick from a distance (Fig.~\ref{fig:failures_material}). The texture and color of different materials can appear different under shadow or extreme light, showing a higher resemblance to another material. For instance, under the shadow, concrete is classified as asphalt (Fig.~\ref{fig:failures_light} - left top). 
%
Moreover, some patterns or objects can visually look similar to certain materials. For example, the model initially classified certain plant pits (Fig.~\ref{fig:failures_material} - left top) or brownish metal covers (Fig.~\ref{fig:failures_material} - left bottom) as bricks alongside the concrete pavement and would incorrectly predict mixed materials for that part of the sidewalk, or even small pieces of broken concrete or granite were classified as cobblestones (Fig.~\ref{fig:failures_material} - left middle). Adding more images with this pattern to the training data improved the model's performance in the next stage. Some correct predictions are highlighted on the right side of Fig.~\ref{fig:failures_material}.
%
The active learning strategy significantly helped with choosing the right data \highlight{at each stage}. Having an expert in the loop to review the results in each stage enabled identifying specific patterns that were not evident by merely analyzing the quantitative metrics of the model. 

\subsection{Challenges}
One of the key challenges of our work was dealing with different textures of the same object (sidewalk). Objects have defined boundaries that are easier to classify~\citep{jain2018recognizing}. However, similar textures can appear on multiple objects. For instance, red bricks are used in both building facades and sidewalk pavings (although different types of bricks are used for each purpose, they possess very close visual characteristics). Our goal is to have a model that can detect \emph{sidewalks} of certain materials from street-view images. \removed{so if we have similar textures on different objects, the model can distinguish between them.} 

Another challenging aspect of this task is the high degree of within-class variation and between-class similarities. For instance, NYC designated five different types of concrete as standard materials for sidewalk pavings, while Boston uses three different types of concrete. Each of these types has distinct visual features that, in some cases, can resemble materials of other classes, which pose further challenges to the classification task. Distinguishing between dark concrete and bluestone in some cases is very difficult, even for humans. When wet, some concretes with aggregates can look very similar to granite, and under the shadow, asphalt and worn-off concrete can look very similar.
%
Having a model that can accurately handle the within-class variability with between-class similarity calls for smartly selected training datasets with a good distribution of different classes as well as multiple variants of the same material under different conditions. 

\begin{figure}[t!]
\centering
\includegraphics[width=0.7\linewidth]{figs/failures_light_compressed.pdf}
\caption{\textbf{Left}: Exposure to direct sunlight changed the appearance of colors and texture of the paving material, \removed{making them resemble another class.} \textbf{Left top}: \removed{asphalt was predicted for the parts in shadow instead of concrete.} \highlight{Part of a concrete sidewalk under the shadow was classified as asphalt.} \textbf{Left bottom}: \removed{Concrete was predicted for the parts of the sidewalk under direct sunlight instead of granite.} \highlight{Part of a granite surface under direct sunlight was classified as concrete.} \textbf{Right}: The correct predictions of the final model in the same settings.}
\label{fig:failures_light}
\end{figure}

\subsection{Limitations} 

Even though CitySurfaces can provide city-scale sidewalk material classification, some challenges remain unaddressed.
%
For instance, in the absence of proper sidewalk network data, it can be challenging to map the materials to their corresponding locations accurately. The maps in Fig.~\ref{fig:overview} are based on the road centerlines where GSV cars traveled to capture images, depicting the dominant materials for each street segment by taking an average over the materials observed in each image from both the left and right sides of the street. 
%
However, knowing the exact location of certain materials is critical for urban designers, planners, and those working with safety and ease of walk for people with special needs. Although our model produces this result at a highly fine level, we cannot depict this variety in detail without proper sidewalk network data. Having separate maps for left and right sidewalks can be one solution, but the intersections where more than one street is captured pose a challenge for assigning the correct materials to each segment. 

Also, street-level images have some inherent limitations. Since the images are taken by cars moving alongside streets, in many instances, specifically in dense urban areas, the cars parked on the sides blocked the sidewalk view, as shown in the first street-view image of Fig.~\ref{fig:gsv-diverse}. The issue can be mitigated to some extent by adjusting the heading and pitch of the camera, but that solution fails in images with large vehicles like trucks, or when the car\hightlight{ with mounted cameras} is too close to the sidewalks. 

==> old/highlights.tex <==



Presents the first study (to our knowledge) that uses deep-learning-based segmentation methods for large-scale localization and classification of sidewalk paving materials.

The framework does not rely on pretrained models, it is trained on the new dataset created using our framework. 

3200 street-level images from Boston and Manhattan were annotated, using CitySurfaces active learning framework to significantly reduce pixel-level annotation costs, and to yield increased segmentation accuracy. 

We show the capabilities of the model to extract surface information from cities outside our training domain for which no ground truth sidewalk surface data exists. 


The model weights and generated datasets are made publicly available. 







==> old/intro.tex <==
% \linenumbers
\section{Introduction}
% \maryam{check the refs style guide in the author's guide to make sure we are following the correct format. Check the electronic art requirements.}

\removed{The surface of cities has gone through tremendous changes since the formation of the early settlements. From stone causeways of ancient Egypt to crosswalks paved with wood planks, flagstones, granite or bricks~\citep{tillson1900street}; from natural soil to impervious concretes and dark, heat-absorbing asphalts of the industrialized cities~\citep{lay2020paving}, to modern permeable materials designed to address water runoff and excessive heat absorption challenges; city pavements evolved through time, responding to the new requirements of each era. However, in the race to conquer more land, the natural environment is put at risk, apart from the economic, social, and public health burdens created by uninformed decisions of the past.  }

\highlight{As urban areas expand around the world, more impervious surfaces replace the natural landscape, creating significant ecological, hydrological, and economic disruptions~\citep{arnold1996impervious, chithra2015impacts}. Choosing the right material to cover city surfaces has become a critical issue in mitigating the adverse effects of increased anthropogenic activities.} 
%
Historically, local availability, cost, strength, and aesthetics were the main factors influencing the choice of \highlight{surface} pavements \citep{lay2020paving}\highlight{\citep{tillson1900street}}. The advent of asphalt and, later, concrete changed the face of cities. The longevity and durability coupled with relatively low production and installation costs made them the pavements of choice. However, as it was later revealed, these benefits came with huge environmental burdens\citep{van2015towards}. \removed{The excessive use of impervious surfaces is shown to be the primary cause of the Combined Sewer Overflows (CSOs), which can lead to massive pollution of natural bodies of water and street flooding~\citep{joshi2021not}. Sidewalk pavements can also create public health hazards such as outdoor falls or pose a barrier to walkability and accessibility of public spaces, specifically for the more vulnerable population and wheelchair users~\citep{talbot2005falls, chippendale2015, thomas2020keep, CLIFTON200795,AGHAABBASI2018475}.}

\highlight{The sharp rise in urban temperature above the neighboring rural areas -a phenomenon called Urban Heat Island (UHI) effect ~\removed{\citep{mohajerani2017urban}} ~\citep{oke1982energetic}- is shown to be directly associated with surface characteristics, such as thermal performance and reflectivity, which can influence micro-climates within the city by absorbing more diurnal heat and emitting that into the atmosphere at nights~\citep{polacco_study_2012, wu2018characterizing, nwakaire2020urban}. Natural surfaces and vegetation increase the amount of evapotranspiration, hence, decrease the overall temperature and create a cool island effect~\citep{amati2010green, du2017quantifying}. Reflective/high-albedo materials are also known to decrease UHI~\citep{akbari2009global, santamouris2011using, santamouris2013using, zhu2019review}. Hence, the spatial distribution of land cover has a strong impact on the surface temperature~\citep{chen2017impacts}. UHI can negatively impact public health, ecological environment, and urban liveability~\citep{estoque2017effects}. }

\begin{figure*}
\centering
\includegraphics[width=\linewidth]{figs/overview_compressed.pdf}
\caption{\removed{Using CitySurfaces to classify paving materials from street-level images of Chicago, Washington DC, and Brooklyn (not part of our training data).
In each city, we collected street-level images at every five meters, covering the whole street network. The maps depict dominant paving materials in each
street segment. Segments where the dominant material differs from concrete are drawn using a thicker line. As can be seen, Washington DC uses
more diverse paving materials compared to Chicago and Brooklyn, where concrete is more widely used. However, downtown Chicago (top left) stands out
from the rest of the city in the way diverse materials such as granite paved the surface of the city.} \highlight{Using CitySurfaces to map the dominant surface material in Chicago, Washington DC, and Brooklyn (not part of our training data). Segments where the dominant material differs from concrete are drawn using a thicker line.} 
}
\label{fig:overview}
\end{figure*}
\highlight{Today, the majority of the urbanized areas are covered with impermeable materials which prohibit the infiltration of the water into the underlying soil, increase both the magnitude and frequency of surface runoffs~\citep{bell2019modeling, shuster2005impacts}, reduce the groundwater recharge, and negatively impact the water quality. The excessive use of impervious surfaces is shown to be the primary cause of the Combined Sewer Overflows (CSOs), which can lead to massive pollution of natural bodies of water and street flooding~\citep{joshi2021not}.}

\highlight{Sidewalks and roads form the main part of the urban ground surfaces. Unlike roads, sidewalks have high variability in color, texture, and types of paving materials. Aside from the mentioned impacts, the choice of sidewalk pavements can also lead to public health hazards such as outdoor falls, or pose a barrier to walkability and accessibility of public spaces, specifically for the more vulnerable population and wheelchair users~\citep{talbot2005falls, CLIFTON200795,AGHAABBASI2018475}. Studies show that uneven surfaces, indistinguishable surface colors, and low-friction materials contribute to the high incidence of outdoor falls in elderly populations~\citep{chippendale2015, thomas2020keep}.}

Despite the substantial economic, environmental, public health, and safety implications of sidewalk pavements~\citep{muench2010greenroads,van2015towards, estoque2017effects}, most cities, even in industrialized economies, still lack information about the location, condition, and paving materials of their sidewalks~\citep{deitz2021squeaky}. The lack of data creates barriers to understanding the real extent of the environmental and social impacts of using different materials and inhibits our ability to take a complex system approach to sustainability assessment~\citep{van2015towards}. For instance, studies show a significant intra-urban variability of the urban thermal environment due to the street-level heterogeneity of paving materials~\citep{agathangelidis2020urban}. However, the data scarcity makes it challenging to measure this variability across different neighborhoods~\removed{ the impact of different pavement materials on
surface UHI} and consequently, \removed{develop}~\highlight{impedes the development of} a sustainable and resilient mitigation response plan~\citep{yang2019local, akbari2008urban, li2013relationship}. In the absence of fine-scale data, studies mainly rely on remote sensing images; however, the high-resolution aerial images are both spatially and temporally sparse~\citep{zhang2009bi}, requiring researchers to use a variety of data aggregation and extrapolation techniques to fill in the missing data, which can~\highlight{lead to high bias and} hurt the validity of the final results~\removed{and lead to high bias}. 

Collecting comprehensive and fine-scale sidewalk data using conventional methods is time-consuming and cost-prohibitive. Recent technological innovations in data collection opened new frontiers for research on public space and pedestrian facilities, creating opportunities to track features of interest at higher temporal frequencies and more granular geographic scales~\citep{glaeser2018big}. 
%
The use of street-level images in urban analysis has gained popularity since the introduction of Google~Street~View~(GSV)~\citep{anguelov2010google} and Microsoft Street Slide~\citep{kopf2010street}, services that provide panoramic images captured by cameras mounted on a fleet of cars. Concurrently, developments in machine learning and computer vision applied to these new datasets have enabled novel research directions to measure the ``unmeasurable'' in urban built environments~\citep{ewing2009measuring}, including sidewalks~\citep{frackelton2013measuring, ai2016automated}.   


In this work, 
%
we address this data gap and take a step towards exploring the surface of our cities through CitySurfaces, a framework aimed at generating city-wide pavement material information by leveraging a collection of urban datasets. 
%
We combine active learning and computer vision-based segmentation model to locate, delineate, and classify sidewalk paving materials from street-level images.
%
Our framework adopts a recent high-performing segmentation model~\citep{tao2020hierarchical}, which uses hierarchical multi-scale attention combined with object-contextual representations.
%
To tackle the challenges of high annotation costs associated with dense semantic label annotation, we make use of an iterative, multi-stage active learning approach, together with a previously acquired sidewalk inventory from Boston, which lists the dominant paving material for a given street segment.
%
We demonstrate how the trained segmentation model can be extended with additional classes of materials with noticeably less effort, making it a versatile approach that can be used in cities with varying urban fabrics and paving materials.
%
To show the generalization capabilities of CitySurfaces, we employ our framework in the segmentation of street-level images from four different cities: Brooklyn, Chicago, Washington DC, and Philadelphia, none of which were included in the training process. Fig.~\ref{fig:overview} highlights how different pavement materials are spatially distributed in three cities.

%
Our contributions can be summarized as follows:
\begin{itemize}[noitemsep]
    \item We present the first study (to our knowledge) that uses deep-learning-based segmentation methods for large-scale localization and classification of sidewalk paving materials.
    \item We adopt an active learning strategy to significantly reduce pixel-level annotation costs for training data generation, and yield increased segmentation accuracy.
     \item We conduct extensive experiments using street-level images from six different cities demonstrating that our model can be applied to cities with varying urban fabrics, even outside of the domain of the training data. 
    \item~\removed{We make the results of our material classification in the six selected cities publicly available} \highlight{We make our model as well as the results of our material classification in the six selected cities, publicly available} (omitted to satisfy double-blind review requirements).

\end{itemize} 


==> old/method.tex <==
\section{CitySurfaces}

\begin{figure*}[h!]
\centering
\includegraphics[width=\linewidth]{figs/pipeline_compressed.pdf}
\caption{\removed{CitySurfaces workflow: \textbf{Block (a):} Creating the initial ground truth labels using the Boston sidewalk inventory and GSV images. A sample of images is chosen and fed to a pre-trained HRNet, which outputs annotation labels containing two classes of interest: roads and sidewalks. The labels are then manually refined so each paving sidewalk material is represented using a distinct color which will form our ground truth set; \textbf{Block (b)} We iteratively choose representative and informative samples to retrain the segmentation model, which can classify five classes of surface materials, plus roads. The model is run on new data, and the segmentation accuracy is used as criteria to guide choosing new samples from Boston and later Manhattan images. In each stage, the most representative and informative test data are chosen, and the annotations are manually refined and added to the training set to retrain the network; \textbf{Block (c)} Introducing three new classes of materials that initially were not part of the Boston inventory, but were among the standard NYC sidewalk materials. The pre-trained model from block (b) is retrained on the newly annotated image data, including the three new classes. The final model can classify eight classes of different materials, including cobblestone streets.}~\highlight{CitySurfaces workflow. Block (a): Creating the initial ground truth labels using the Boston sidewalk inventory and GSV images. A sample of unlabeled images
is fed to a pre-trained HRNet, which outputs annotation labels containing two classes of interest: roads and sidewalks. The labels are manually refined to represent the five sidewalk paving classes, forming our ground truth set; Block (b): Training the base model to classify five classes of surface materials, plus roads. The data from block (a) is used for the first stage of training. The model is then iteratively retrained for multiple stages on new samples. In each stage, the most representative and informative samples are chosen, and the annotations are manually refined and added to the training set to retrain the network; Block (c): Introducing three new classes of materials. The pre-trained model from block (b) is retrained on the newly annotated image with three new classes. The final model can classify eight classes of different materials.}}


\label{fig:workflow}
\end{figure*}


CitySurfaces adopts an active learning approach for the semantic segmentation of sidewalk paving materials. Using this framework, we aim to: 1) Train a model that can classify five different paving materials plus asphalt roads; 2) Extract information about sidewalk materials of a city for which no ground truth sidewalk inventory exists (e.g., NYC); and 3) Extend the model to classify additional classes of materials so that it can be applied to a more general set of cities.

Active learning aims at achieving high accuracy while minimizing the amount of required labeled data. The main hypothesis is, if we allow the model to choose the training data, it will perform better with fewer labeled instances~\citep{settles2009active}. Through iteratively selecting the most informative or representative images to be labeled, fewer labeled instances are required to achieve similar performance compared to randomly selecting a large sample as training data and annotating all of it at once \citep{bloodgood2014method, huang2010active}. 

In general, our multi-stage workflow is different from previous works in active learning for semantic segmentation in two important ways: First, our sample selection method is not fully automated; we use the uncertainty measure to filter our pool of unlabeled data in each stage, but we also use domain expertise for selecting a sample of images to be annotated and added to the training set in the next stage.
%
Second, our query frequency is ten epochs (each epoch is a pass through all training data). The conventional approach in active learning is to select new samples (query) every iteration, which can work in cases where the cost of annotation is not high or in experimental studies that work with already annotated images to advance the field and develop new query algorithms, as is the case with most of the already published works in active learning for semantic segmentation, where they use datasets such as CityScapes~\citep{cordts2016cityscapes} or ADE20k~\citep{zhou2017scene}. However, since no annotated dataset exists for sidewalk materials, we have to annotate every new sample we choose during the training process, and it is impractical to annotate a new sample for every iteration~\citep{kim2020message}. To overcome this, we adopt a multi-stage framework and annotate a new sample at the end of each stage, where each stage consists of ten epochs.


Our workflow has three major blocks as illustrated in Figure~\ref{fig:workflow}: Block (a) creating initial training labels; Block (b) training a material segmentation model and; Block (c) extending the model to segment three additional classes from NYC standard materials. In this section, we first describe the different blocks of our workflow in detail, followed by a description of the semantic segmentation model.

\subsection{Block (a): Initial image annotation}

To start the training process, we need a set of annotated images. To obtain the annotated data, we randomly sample 1,000 images from a pool of unlabeled Boston street-level images and feed that sample into HRNet-W48~\citep{sun2019high, wang2020deep} model pre-trained on Cityscapes~\citep{cordts2016cityscapes} and get the initial segmentation results (Figure~\ref{fig:workflow}(a)). The model outputs 19 classes from which we only keep roads and sidewalks. 
%
To generate an initial set of labeled data, we make use of the Boston Sidewalk Inventory (detailed in Section~\ref{data:boston}). We first query for the street segments of the images in our initial sample and modify the label to match the audited pavement from the inventory. Effectively, we are ensuring that, instead of having a general \emph{sidewalk} class outputted by the pre-trained HRNet, our image set will have annotations according to the ground truth inventory data (e.g., concrete, bricks).
%
We then manually refine them to account for the pre-trained model's prediction errors. In the initial training set, we restrict our sampling to images where the sidewalks mainly consist of a single material and eventually move to more complex material configurations in later stages. The final annotated images were split into 80\% training and 20\% validation to train the model in block (b). 

\subsection{Block (b): Model training on Boston and NYC}
\label{blockb}
In the second block of our framework (Figure~\ref{fig:workflow}(b)), we train an attention-based model (detailed in Section~\ref{model}) using the labeled images from block (a). Our training step initially uses 800 images for training, and 200 images for validation, with a batch size of 8 (2 per GPU), SGD for the optimizer, momentum 0.9, weight decay $5e^{-4}$, and an initial learning rate of 0.002. 
%
We train our model in a multi-stage framework, where each stage consists of ten epochs. In each stage, we choose the epoch with the highest mIoU on the validation set.
%
At the end of each stage, we make two decisions: 1) we select the best model considering all epochs of the current stage; and 2) we analyze the quantitative and qualitative results of the model to guide our sampling of \emph{new} training data. In particular, we analyze the confusion matrix, similarity matrix, as well as the top 10\% of predictions with the highest mIoU and the top 20\% of failures, obtained from the validation phase of the best epoch.
%
The weights of the best model in the current stage are then used to initialize the model in the next stage with more training data. This restating scheme of SGD with the best solution of the previous stage is useful in increasing the chances of finding better solutions in the current stage.


To sample new images, we employ two strategies: i) Uncertainty in predicting unlabeled images: We make use of the model's uncertainty estimations on unlabeled data and select the images that were most challenging for the model to predict; and ii) Performance on validation set: By examining per-image IoU, uncertainty, and error rates of the images from failure and success cases together with confusion matrices, we construct a set of sample images to be used as inputs for finding similar unlabeled images. A more detailed explanation of these two techniques is provided in~\ref{appendixa}. 

\begin{figure}[t!]
\centering
\includegraphics[width=0.5\linewidth]{figs/new_mat.pdf}
\caption{Examples of how the annotation labels with additional classes were created from the output of the model in block (b) of our framework. The model trained in block (b) classified granite blocks and cobblestone as background, leaving smooth and clear boundaries, which helps to augment the labels with new classes during manual refinement and train a model that can classify eight different materials (block (c) of the framework).}
\label{fig:newmaterials}
\end{figure}

Following the sample selection strategies, we retrieve 300 unlabeled images, apply the current model on these new unlabeled images to generate a prediction, and then modify the predicted labels to add them to the overall training set, such that the segmentation model has access to more samples of hard-to-segment images. To improve model generalization, in the third stage, we begin including images from Manhattan, which has a different urban fabric and more diverse forms and types of paving materials, in our pool of unlabeled data. Since no ground truth data exists for Manhattan, to create the ground truth label, we need to have a model with reliable performance to create the base annotation. We chose the third stage since the model reached a reliable performance (83\% mIoU) in detecting the main classes, and outputs had clear borders compared to the other two stages. The selected images from Manhattan were fed to the model, and the results were corrected and refined using feedback from the domain expert and added to the training dataset. 
%
The segmentation model is then trained on the combined set of the initial and newly annotated data (1,100 images), initialized with the weight from the best epoch of the previous stage. This procedure is iterated for five stages (at which point we observe no further notable improvements). The model at the final stage was trained on 2,500 images (Figure~\ref{fig:workflow}(b)), and achieved 88.6 \% mIoU on a held-out test set. 


\subsection{Block (c): Including additional materials from NYC}
\label{block(c)}

Once the model in block (b) attains sufficiently accurate segmentation performance, we extend it by adding three additional classes (Figure~\ref{fig:workflow}(c)). The three additional classes are granite blocks, hexagonal pavers, and cobblestone. These materials are standard sidewalk materials in the NYC street design manual~\citep{new2020street}. While granite blocks and cobblestones were also observed in Boston, they were not included in the Boston sidewalk inventory. Since the original model in block (b) was not trained to detect these materials, they are initially either classified as background (mostly granite blocks and cobblestones) or misclassified (mostly hexagonal pavers) as other visually similar materials. To collect street-view images that have these new materials, we follow the NYC and Boston street design manuals \citep{bostoncomplete,new2020street} to filter unlabeled data from the locations in which these materials can be found. For example, hexagonal pavers (NYC only) are typically used on sidewalks adjacent to parks and open spaces, and cobblestones are used in historic districts. 

We select a total of 800 images that contain these new classes to be iteratively sampled for training, 150 additional images for the validation set, and 200 images for the held-out test set. Annotating the new image set consumed fewer resources as compared to the initial annotations since smooth model predictions typically leave clear boundaries, which only needed to be assigned the appropriate label (see Figure~\ref{fig:newmaterials}). The newly generated set of labels was used to train the model by initializing the architecture with model weights in block (b) and only replacing the final softmax layer instead, to produce ten output channels (corresponding to eight paving materials, plus the road, and background). At the end of each stage, we select a new sample of unlabeled images following the same process explained in Section~\ref{blockb}, run them through the model, obtain segmentation predictions, refine the results, and retrain the model. In total, 726 additional images were added to the training set, and in the final stage, the model was trained on 3,226 images (2,500 from block (b) + 726). We halt training in stage 3, after 30 epochs (Figure~\ref{fig:matrix} stage 3), and test the model on the held-out test set~(Figure~\ref{fig:workflow}(c)). Figure~\ref{fig:matrix} visualizes confusion matrices for all three stages of our extended model, illustrating model performance as a function of the amount of training data. These matrices were also used in part to guide the sampling of images to annotate. 

\begin{figure*}
\centering
\includegraphics[width=1.0\linewidth]{figs/matrix_compressed.pdf}
\caption{Confusion matrix for the three stages of the extended model. These results guided sample selection and signaled which type of images should be included in the training data for the next stage. Notice the improvement of the predictions for hexagonal pavers, granite block, and granite/bluestone (highlighted in red).
}
\label{fig:matrix}
\end{figure*}


\begin{figure}[h!]
\centering
\includegraphics[width=0.5\linewidth]{figs/evolution_compressed.pdf}
\caption{Evolution of the block (c) extended model's inference through different training stages.}
\label{fig:cycles}
\end{figure}


Using the described method, model performance increases from 74.3\% mIoU to 88.6\% for the base model (block (b)) and to 90.5\% in the extended model (block (c)), with the manual refinement time decreasing from 25 to 4 minutes per image. Figure~\ref{fig:cycles} depicts the evolution of the segmentation results of block (c) through the active learning stages. The model outputs more refined boundaries and significantly less noise in later stages; thus, significantly less time is needed to modify the newly annotated data as the stages go on. In each stage, the model is initialized with the weights from the previous stage. 


\subsection{Semantic segmentation model} 
\label{model}

For our semantic segmentation task (blocks (b) and (c)), we adopt the Hierarchical Multi-Scale Attention~\citep{tao2020hierarchical} and fine-tune the parameters on our dataset. To train the model, following~\citet{zhu2019improving}, we employ class uniform sampling in the data loader, which chooses equal samples for each class for handling our class imbalance, since some classes like road and background are almost present in all images, whereas classes like cobblestone and hexagonal pavers are not that prevalent. 
%
The Region Mutual Information (RMI) loss \citep{zhao2019region} was employed as the primary loss function.  RMI takes the relationship between pixels into account and uses the neighboring pixels around each pixel to represent it instead of only relying on one pixel to calculate the loss. We run our experiments with and without the RMI loss function for the main segmentation head. In the absence of RMI, standard cross-entropy loss was used instead. The model under the same setting but without RMI loss performed slightly worse (89.84) compared to the one where RMI loss was used (90.51). Figure~\ref{fig:attention} presents an overview of the architecture. Next, we describe the network's architecture in more detail.


\begin{figure}[h!]
\centering
\includegraphics[width=0.5\linewidth]{figs/flowchart.pdf}
\caption{The general architecture of the hierarchical multi-scale attention (HMSA) based semantic segmentation method \citep{tao2020hierarchical}. The inputs are images from two scales. The network learns the relative attention between scales and hierarchically applies the learned attention to combine the results from two segmentation heads and make a prediction.}
\label{fig:attention}
\end{figure}



\subsubsection{Backbone}
\label{hrnet}
We chose HRNet-OCR \citep{yuan2019object} as the backbone. The network comprises of HRNet-W48~\citep{sun2019high,wang2020deep} and adds Object-Contextual Representations \citep{yuan2019object} to further augment the representation extracted by the HRNet. The final representation from HRNet-W48 works as the input to the OCR module, which computes the weighted aggregation of all the object region representations to augment the representation of each pixel. The weights are calculated based on the relations between pixels and object regions. The augmented representations are input for the attention model described next. 

\subsubsection{Attention Model}

The model is mainly based on Share-Net \citep{chen2016attention}. Suppose an input image is resized to several scales, i.e., $s \in \{ 1,...,S\}$. Each scale is passed through the backbone part (HRNet-W48+OCR), and we can get the output feature $f_{i,c}^s$. For the feature, $c \in \{1, ..., C\}$ ($C$ is the number of classes of interest, and $i$ ranges over all the spatial positions). As shown in Figure~\ref{fig:attention}, the features then go through two heads, one for attention generation and the other for segmentation. The features $f_{i,c}^s$ are resized for different scales to have the same resolution (with respect to the finest scale) using bilinear interpolation before passing the model heads. For the attention head, we generate the learned weights for $f_{i,c}^s$ which is represented by $a_{i,c}^s$. This weight is integrated into the initial output $h_{i,c}^s$ from the segmentation head, and we have:

\begin{equation}
    g_{i,c}^s = a_{i,c}^s * h_{i,c}^s,
\end{equation}
in which $g_{i,c}^s$ is the final output score map for scale s, and $*$ here represents the pixel-wise multiplication.


In the model, the combination of score maps is similar to \citep{tao2020hierarchical} to make the flexible scales during inference time possible and improve the training efficiency. During the training, we only need to train with two adjacent scales (as shown in Figure~\ref{fig:attention}). During testing, weights for the network are shared for each adjacent scale pair.

To be more specific, suppose the two selected adjacent scales are $1x$ and $0.5x$ (the final selected scales during training in the model are $0.5x$, $1x$, and $2x$) to obtain the pair of scaled images for the model input. For inference, we can hierarchically and repeatedly use the learned attention to combine $N$ scales of predictions together. Precedence is given to lower scales since they have a more global context and can choose where predictions need to be refined by higher scale predictions. The final combination principle for these adjacent scales is defined as:
\begin{equation}
    g_{i,c} = a_{i,c}^0.5 * h_{i,c}^0.5 + (1-a_{i,c}^0.5)* h_{i,c}^1,
\end{equation}
The hierarchical mechanism used in the model coupled with the powerful HRNet-OCR backbone provides a robust architecture for the challenging task of material classification \emph{in the wild}. 
% 


==> old/notes.tex <==
%
% City agencies need to have detailed information about different types of materials in each street segment for maintenance planning, assessing ADA compliance, and aiding with stormwater runoff management \citep{wang2019impacts, lawsuit}. Environmental agencies concerned with reducing the urban heat island effect require this information for analyzing the impact of different pavements as well as replacement planning and prioritizing \citep{pomerantz1997paving, santamouris2012using, hendel2018pavement}. Having data about surface materials is of critical importance in route planning and fall prevention programs run by occupational therapists, and individuals or organizations working with the disabled and elderly people \citep{chippendale2015, lee2018impact, chippendale2020outdoor}. Despite the crucial need to have detailed datasets about sidewalk materials, few cities maintain such spatial catalogues.

% The limited datasets that do exist are mainly restricted to describing the dominant material of a given segment rather than providing detailed information on how different types of paving materials are spatially distributed.  

% Sidewalk pavements can also impose public health hazards such as outdoor falls \citep{?}, or become a barrier to walkability and accessibility of public spaces, specifically for those with movement or vision impairments \citep{?}. 



%%%%%%

discussion 


%The distance of the sidewalk from the camera (mostly in the images from right side of the streets) plays a key role in model performance as well. Sidewalks located further from the camera are more difficult to classify, since the texture, color scheme, and the borders of the finer objects like granite blocks and stones are more difficult to detect. We plan to introduce some constraint for the bounding box of detected sidewalks and further modify our GSV queries by adjust the camera settings based on some distance features to mitigate the problem. 
% \fabio{I think that this should be re-written as to make sure it reads as a data problem and that we have mitigated the issue somehow -- but that further work needs to be done to improve the model even more.}




% \begin{figure}[h!]
% \centering
% \includegraphics[width=\linewidth]{figs/CRF5.png}
% \caption{Results of applying CRF post processing to the model predictions.}
% \label{fig:CRF}
% \end{figure}

% % Besides the mentioned challenges, we will also consider the improvement of post image processing to eliminate noises in our segmentation results. We want to refine the coarse output based on the label at each location itself, and the neighboring positions’ labels and locations. Such spatial correlation in label domain is not well considered in our MaterialNet. We have introduced the most prevalent Conditional Random Filed (CRF) \citep{wallach2004conditional, yuan2020structpool} to achieve this goal. The basic idea for CRF is to construct the label assignment as an energy minimization problem. This method assigns the most probable label to each location in the image to achieve lower energy, and thus, higher segmentation accuracy. To be more specific, CRF is made up of two terms, the unary energy term, and the pairwise energy term \cite{wallach2004conditional}. The first one will increase if the label assignment disagrees with the initial classifier, while the second one will punish the case if two similar/neighboring pixels have different labels. Several visualized examples of results for such methods can be found in Fig. \ref{fig:CRF}. As can be found in the first row of the figure, the details of bicycle are better preserved and refined with the CRF model. Such details are even missed in the ground truth. This is because the effects of pairwise energy term, which unify the labels of pixels with similar RGB values. The second advantage can be found in the second and the third row, in which we can find a small area of wrong labels are eliminated. As the pairwise energy term will further judge the pixel label with its neighbors and smooth the segmentation results, the noise area is eliminated. 

% However, we have to mention that the drawback of such method. Its performance heavily relies on the initial segmentation results. The wrong annotations will also spread if the initial segmentation performance is poor. To avoid such drawback, for the future work, we will propose an new integrated way for MaterialNet and CRF to jointly optimize the pixel-level data feature and spatial correlation.  









% imaged under different viewing directions 

% “surface texture, geometry and lighting conditions
% associate each pixel of an image with a categorical label.
% inherent spatial dependency 



% “in the wild” where imaging conditions such as lighting color and direction, orientation, sensor type, etc., are unpredictable





 






%Boston : (Smooth finish cast-inplace concrete, Dark aggregate and/or exposed fine aggregate concrete) 
%Dark aggregate and/or exposed fine aggregate concrete

%Manhattan: Unpigmented Concrete - Pigmented Concrete (Dark) Silicon carbide - Pigmented Concrete
%(Historic Materials) - Concrete with Exposed Aggregate - Concrete with London Paver Scoring - 
  




% - The context dependency when using OCR and how to overcome it ? (at second stage, the model predicted all the sidewalks between two green ribbons as asphalt - adding more examples with different contexts helped ) 





































\subsection{mixture of everything from UHI papers} 


sustainable cities 



Paving materials have strong implications for sustainability, spanning from economic to natural environment and social well-being \citep{muench2010greenroads,?,?}. Having the highest variety of materials used for surface pavements, sidewalks can play a major role in 

Choosing the proper material for sidewalk pavement goes beyond the durability or monetary costs of production, installation, and maintenance. These factors, although critical, do not reflect the environmental externalities pavement materials can create. 
 






sustainability rating system for sidewalks and paving material is the most important element of sidewalks in that context. 

``walking is the broadly accessible mode of sustainable transportation and safe recreation while facilitating commercial and social exchange and encouraging citizens to be physically active.

Pedestrian pavements are therefore designed to be technically, economically and aesthetically suitable for users. The design process, however, fails to apply comprehensive life cycle environmental data to identify suitable construction solutions and urban management strategies that contribute to minimizing environmental impacts. \citep{mendoza2012planning}"

\textbf{Very important \citep{takebayashi2014study}}


green / sustainable infrastructure

sustainable pavement \citep{al2021sustainable} :
``Artificial and man-made pavements have been recognised as one of the major origins that deteriorate the thermal environments for living.
\newline

The lack of sustained operation and maintenance programs among local government agencies is mentioned as the main reason behind the poor quality of pedestrian infrastructure \citep{patel2019economic}

Using sustainable materials means consuming less amount of energy in production \cite{?}, using recycled solid waste materials as a coarse aggregate \cite{najjar2016green}, using porous materials that can help with water run-off management as well as surface water infiltration \cite{}, 



examples: 
1) 
\citep{zhao2014strong}  \textit{Rural pixels are classified in the MODIS land cover map as natural surfaces such as forests, grassland, cropland and bare soils. To avoid high bias of UHI, we excluded water pixels. Urban pixels are classified in the MODIS land cover map as urban and built-up surface.}

land surfaces are categorized into five land units: vegetation, glacier, wetland, urban and lake. Each grid cell can have one or more of these land units. The surface radiation and energy balance equations are solved separately for these land units, and the results are aggregated to yield grid cell means. Specifically, the urban land unit is modelled using a `canyon' structure and consists of the following subsurfaces: roof, sunlit wall, shaded wall, and pervious (for example bare soil) and impervious (for example road, sidewalk and car park) canyon floor.


 We note that even at this finest resolution the grid cell is still large enough that the total urban area in a grid cell can be a combination of several urban areas. The surface skin temperature was determined from the emitted long-wave radiation for each land unit, with an emissivity of 0.88 for the urban land unit and 0.96 for the vegetated land unit. The urban emissivity is the mean value of the weighted averages of the emissivity values of the urban subsurfaces prescribed in the model for the selected cities. The rural emissivity is the mean value of the weighted average of the vegetation and soil emissivity.
 

2) 
\cite{Herath2021} : This study used the TAPM mesoscale climate model (Hurley, Physick, \& Luhar, 2005) 
TAPM employs a tiled or mosaic approach where the surface temperature is comprised of three different land-use types. These three types are the urban impervious surfaces (a combination of roofs, roads and walls), the vegetation coupled to the urban street canyon (referred to as inside-canyon vegetation) and a separate vegetation tile that does not directly couple to the urban surfaces that represents natural vegetation as well as large parks (referred to as outside-canyon vegetation). The combined area fraction of the urban impervious surfaces with the inside-canyon vegetation. The surface temperature for the urban area TU is calculated from the combined outgoing longwave radiation of both the impervious surfaces and the inside-canyon vegetation (Thatcher \& Hurley, 2012).
which is dynamically coupled with the UCLEM urban canopy scheme for urban parameterization. By comparing the performance of a broad range of urban surface characteristics at a large metropolitan area, our results can be used to inform urban cooling strategies and adaptation planning. This will in turn help build a heat-resilient and livable city of Melbourne as well as other cities with a similar temperate oceanic climate.


\citep{zhou2019satellite} 
Satellite remote sensing of surface urban heat islands

\maryam{ from Nasa proposal :  As climate change unfolds on a global scale, cities must adapt to the realities of extreme heat, particularly heat due to the Urban Heat Island (UHI) effect. Cities that experience the UHI are substantially warmer than their surrounding rural areas due to impervious ground cover that prevents evaporative cooling as well as due to the complex-built environment that absorbs and retains more solar energy than natural areas.
%

Since traditional meteorological techniques are inadequate to account for the complexities associated with the surface heterogeneity that accurately quantify the urban land-atmosphere interactions at the neighborhood scale for fine spatial and temporal resolutions, satellite remote sensing techniques are needed. However, satellite images have different spatial and temporal resolution which require extensive validation and calibration. Some have high spatial but low temporal and vice versa.

The inadequacy of characterizing the urban land surface temperature at the neighborhood scale diurnally is apparent from the figure. High spatial and temporal resolutions are needed to capture the local heterogeneous urban heat island effects, and urban heat storage with direct applications to scientifically assessed climate change adaptation and mitigation strategies for urban areas. One way to overcome this deficiency is to develop downscaled LST estimates at finer spatial and temporal resolutions.

to measure LST data from various typical surfaces with high heat storage in the urban environment. These surfaces include impervious asphalt, concrete, rooftops, grass, bare soil, and tree canopy, under both shaded and unshaded conditions. 

calculate spatial correlation between the coincident satellite and ground data.  }


\textbf{what are the implications of lack of fine level data ? }

\citep{coseo2019accurate} : importance of including obscured impervious surfaces in urban heat island models 

\citep{estoque2017effects} : Effects of landscape composition and pattern on land surface temperature

\textbf{Sustainability}: 
To achieve sustainable urban development, performance-based approaches can be used to better understand local land use (Baker, Sipe, \& Gleeson, 2006). Optimizing the urban form can mitigate the impact of future urban heat islands (Yin, Yuan, Lu, Huang, \& Liu, 2018). 

The current study incorporates sustainability goals with smart city initiatives. 

Sustainability goals can be often overlooked 


% To address the market failures\maryam{add def} that create environmental externalities \maryam{add def} 

UHI can adversely impact the sustainability of regions by increasing the dependence of mechanical cooling which results in increased greenhouse gas emissions, consumption of water in the thermoelectric process and increased costs of living for regional residents. The UHI can also increase the incidence and severity of heat related illnesses as well as alter sensitive ecological systems. 


\textbf{Impact on UHI}: 

Impact of the spatial distribution of land cover on surface temperatures (Chen \& Zhang, 2017). 
The surface temperatures of urban construction coverage are high, and those of vegetation coverage are low (Zhou, Huang, \& Cadenasso, 2011). 

In megacities, which have relatively high and low temperatures, it is extremely important to conduct local climate classification studies. Local climate zone classification uses a combination of four different indices: urban structure, surface cover, urban texture, and anthropogenic heat sources (Oke, Mills, Christen, \& Voogt, 2017; Stewart \& Oke, 2012). 


The design process, however, fails to apply comprehensive life cycle environmental data to identify suitable construction solutions and urban management strategies that contribute to minimizing environmental impacts.
\cite{gao2019enhanced} The urban expansion with conversion of natural/vegetated cover to artificial surfaces has been broadly recognized as the main contributor to greater UHI effect in most cities (Imhoff et al 2010, Zhou et al 2015, Hu et al 2017, Liet al 2017).

The effects of urban structures and heavy usage of building materials (e.g. concretes and asphalts) on the land surface radiation budget and energy balance, which reduce the latent heat flux and increase the sensible heat flux (Oke 1982, Arnfield 2003). 

the heat released to the air from the urban surface was the major contributor to the increased temperature at nighttime. 


the contribution of urban surface parameters (USPs) for urban heating. 
The importance of city-scale implementation of USPs change to achieve maximum effectiveness in heat reduction \cite{Herath2021, agathangelidis2020urban}


Extreme urban heat, influenced by surface characteristics, negatively affects human thermal comfort. The thermal behaviour of different urban surface parameters (USPs) at large spatial scales is essential for strategic heat mitigation. 

 Urban surfaces are created by converting natural vegetative surfaces into built-up areas (Bai, Chen, \& Shi, 2012; Chen et al., 2015; Ren, 2015; Zhao, 2018). Such large-scale urbanisation subsequently impacts the regional microclimate by exacerbating the urban heat island effect (Gao, Hou, \& Chen, 2019; Li, Schubert, Kropp, \& Rybski, 2020; Zhang, Shou, \& Dickerson, 2009; Zhou, Rybski, \& Kropp, 2017). 


surface emissivity
surface temperature 

and a well-known consequence of urbanization is the urban heat island (UHI), referring to the phenomenon that cities are typically warmer than the surrounding rural areas.

The UHI effect has important implications for energy consumption, air quality, and urban ecosystems. It can also synergistically interact with heat waves and increase morbidity and mortality risks.

This temperature difference can be based on either surface temperature or air temperature.  surface temperature and refer to the UHI as the “surface UHI.

\cite{imhoff2010remote}:
but comparisons across different urban areas have been hampered by the lack of objectively quantifiable and commonly agreed upon definitions for urban density, and urban versus non-urban area. 
The development of impervious surface area (ISA) data derived from 30 m Landsat ETM+ and IKONOS imagery (Yang et al., 2002, Homer et al., 2004) is a reasonable solution providing a continental-wide map of impervious surface fractional areas. 

The ISA data estimate the relative amount of impenetrable surface area, such as pavements for roads and parking lots and roofing materials which in aggregate have been identified as a key environmental indicator of urban land use and water quality (Arnold \& Gibbons, 1996). The ISA data have been used successfully in combination with other comparable resolution remotely sensed data of land surface temperature and vegetation indices to characterize temperature differences (Xian and Crane, 2005, Yuan and Bauer, 2007).






\subsection{Water Runoff}

1)sustainable water filtration
2)detecting streets most susceptible to flooding 
3)prioritize planning for water-runoff management 


percolation or infiltration of stormwater through the surface into the soil below where the water is naturally filtered and pollutants are removed. In contrast normal pavement is an impervious surface that sheds rainfall and associated surface pollutants forcing the water to run off paved surfaces directly into nearby storm drains and then into streams and lakes.


What are the Potential Benefits of Permeable Pavement?
General hydrologic benefits

Permeable pavements help reestablish a more natural hydrologic balance and reduce runoff volume by trapping and slowly releasing precipitation into the ground instead of allowing it to flow into storm drains and out to receiving waters as effluent. This same process also reduces the peak rates of discharge by preventing large, fast pulses of precipitation through the stormwater system.
Permeable pavement can reduce the concentration of some pollutants either physically (by trapping it in the pavement or soil), chemically (bacteria and other microbes can break down and utilize some pollutants), or biologically (plants that grow in-between some types of pavers can trap and store pollutants).
By slowing down the process, permeable pavements can cool down the temperature of urban runoff, reducing the stress and impact on the stream or lake environment.
By controlling the runoff at the source, such as a parking lot, permeable pavement can also reduce the need for or the required size of a regional BMP, such as a wet detention pond, which saves money and effort.
Cold-weather benefits

Another benefit of permeable pavement is the reduced need to apply road salt for deicing in the winter time. Researchers at the University of New Hampshire have observed that permeable asphalt only needs 0 to 25% of the salt routinely applied to normal asphalt (Houle and others, 2009). 
Other researchers have found that the air trapped in the pavement can store heat and release it to the surface, promoting the melting and thawing of snow and ice (Roseen and others, 2012).






==> old/related.tex <==
\section{Literature Review}

\subsection{Sidewalk Pavements}
\label{sidewalk-mat}

 pedestrian facilities can impact the  The paving material of sidewalks can impact the accessibility of public spaces \citep{?}, the ease and comfort of walking, the frequency of required maintenance, and the risk of accidents \cite{thomas2020complexity, ?, ?}. 



It can influence land surface temperature and consequently, UHI \citep{?}, 

urban surface parameters (USPs) 


The Federal Highway Administration detailed some basic requirements and recommendations for designing pedestrian facilities \citep{FHWApeds} and listed concrete as the most widely used paving material, due to its lower cost, longer life time, and versatility of shape, form, color and texture. Moreover, concrete is shown to be a preferred material for minimizing long-term primary energy demand and global warming potentials of urban areas \citep{mendoza2012planning, sousa2019pedestrian}.

However, the impermeable surface of concrete poses some significant challenges in high precipitation areas. Hence, recent works have focused on permeable pavements and porous concretes to manage water runoff, reduce peak swear discharge, increase infiltration and reduce the likelihood of ponding or black ice~\citep{li2017research, wang2021water, chen2017environmental, qiu2020rainfall}.



NYC has recently added permeable interlocking concrete paver (PICP) as an standard materials ~\citep{new2020street}. Most cities publish street design manuals in which standard paving materials are recommended based on the  the sidewalk zone (e.g. furnishing or pedestrian through), fabric (e.g. historic) and landuse. 


% The surface material is of critical importance in the objective assessment of sidewalks \citep{ferreira2007proposal,maghelal2011walkability}. 

The type, color, texture, size, design, cut, and chamfer of paving material can influence found uneven and bumpy surfaces to strongly correlate with walking unsteadiness by comparing surfaces including bricks, cobblestone, and flagstones. Uneven surfaces, indistinguishable surface colors, and low-friction materials contribute to the high incidence of outdoor falls in elderly populations~\citep{talbot2005falls, chippendale2015, thomas2020keep, CLIFTON200795,AGHAABBASI2018475}.
% According to \citet{ferreira2007proposal}, pavement condition and material composition, are critical factors impacting the accessibility level of sidewalks for wheelchair users. 



\maryam{add urban heat Island effect here}

Studies show a significant intra-urban variability of urban thermal environment due to the street-level diversity of surface covers \citep{agathangelidis2020urban}, highlighting the dire need for developing locally-adjusted UHI adaptation strategies.  Lack of fine-level surface cover data at city-scale makes it challenging to draw a realistic picture of the actual extent of this variability across different neighborhoods, measure the impact of different pavement materials on UHI and consequently, develop a sustainable and resilient mitigation response plan \citep{yang2019local}.

% The inadequacy of characterizing the urban land surface temperature at the neighborhood scale diurnally is apparent from the figure. High spatial and temporal resolutions are needed to capture the local heterogeneous urban heat island effects, and urban heat storage with direct applications to scientifically assessed climate change adaptation and mitigation strategies for urban areas. One way to overcome this deficiency is to develop downscaled LST estimates at finer spatial and temporal resolutions.


% The thermal properties of urban materials can lead to a stronger heat storage uptake during daytime and to a gradual heat release at night, maintaining a positive sensible heat flux \cite{?}

% Low vegetation density is responsible for reduced latent heat flux and evapotranspiration cooling \cite{?}

% Anthropogenic heat releases provide additional input to the Surface Energy Budget (SEB) \cite{?}


This meant that the improvement of the thermal environment of the pedestrian space was remarkable. \cite{takebayashi2014study}


\cite{agathangelidis2020urban}
Current practices in UHI calculation mainly rely on remote sensing images to calculate the UHI, however, the high resolution aerial images are both spatially and temporally sparse \citep{?}, requiring researchers to use variety of data aggregation and extrapolation methods to fill in the missing data which can hurt the validity of the final results and lead to high bias level \citep{?}. Recent studies tried to overcome such biases by using drones or other equipment to collect ground level data to be used in combination with the available satellite data as a way to validate and calibrate those and build models to estimate the UHI for the places where no data is available. \citep{?} 



Impact of the spatial distribution of land cover on surface temperatures (Chen \& Zhang, 2017). 
The surface temperatures of urban construction coverage are high, and those of vegetation coverage are low (Zhou, Huang, \& Cadenasso, 2011). 

In megacities, which have relatively high and low temperatures, it is extremely important to conduct local climate classification studies. Local climate zone classification uses a combination of four different indices: urban structure, surface cover, urban texture, and anthropogenic heat sources (Oke, Mills, Christen, \& Voogt, 2017; Stewart \& Oke, 2012). 




build a heat-resilient and livable city
for well-planned adaptation and mitigation responses


Due to its adverse impacts on urban ecological environment and the overall livability of cities, the urban heat island (UHI) phenomenon has become a major research focus in various interrelated fields, including urban climatology, urban ecology, urban planning, and urban geography.
 
% Almost all cities in the united states have a list of standard pavement materials for sidewalks. Various studies have been conducted to calculate the heat budget of various surface materials \cite{?}. Having a database describing the spatial location of each material combined with the fine level shadow accumulation data \cite{?} can provide a highly precise method for the large-scale measurement of the UHI at fine level. 
% Majority of the current work rely on aggregation of the surface type to pervious and impervious / surfaces using the remote sensing images and landsat or NDVI (?) data (30 m?) 



Most cities publish street design manuals in which standard paving materials are recommended based on the  the sidewalk zone (e.g. furnishing or pedestrian through), fabric (e.g. historic) and landuse.

for instance, in raster analysis, pixels belonging to rural areas are often classified as natural surfaces and urban areas are classified as build-up surfaces \citep{zhao2014strong}, treating all different types of urban surfaces, from asphalt to pervious bricks, and reflective granite, porous materials, light and dark materials,  all as having the same heat capacity \maryam{check the ``heat capacity".} 





``the change in its temperature (most often surface temperature) over time as influenced by properties of the paving materials (e.g. albedo, thermal emittance, thermal conductivity, specific heat, and surface convection) and by the ambient environmental conditions (sunlight, wind, air temperature)." 


``Solar reflectance of paved surfaces can be a strong contributor to pavement warming and this warming has the potential to impact the UHIE in those built environments that experience hot weather and are large enough to generate a heat island. "







the need for street-level images and fine-scale analysis of urban heat island 


heterogeneous surface cover 


``remote sensing enables thermal observations with large spatial coverage and
allows the retrieval of the radiometric surface temperature, or as it is typically referred to, the Land Surface Temperature (LST)"


\subsection{from original paper}



% Finding sustainable, resilient solutions to the emerging challenges requires analyzing the roots and drivers of urban changes as well as a close study of the interactions between different parts of the system; a 

% been a major barrier to creating  \cite{yang2019local}
% Lack of fine-scale, comprehensive data describing sidewalk paving materials has been holding researchers back from developing accurate city-wide models to estimate UHI, accounting for the heterogeneity of paving materials. 





UHI refers to the rise in the temperature of metropolitan areas compared to their surroundings, which are often called “cool seas” \citep{?}. Different surfaces have different thermal performance \cite{?},  Darker surfaces like rooftops and roads that absorb heat from sunlight during the day and re-radiate it as thermal radiation at nights \citep{frumkin2016urban, ?}. The lack of trees, vegetation and green spaces that cool the air through evapotranspiration is the second \citep{bhatta2010analysis}, this resulted in .... as well as increasing the energy demand for space cooling \citep{li2019urban}. 

Extreme urban heat, influenced by surface characteristics, negatively affects human thermal comfort. The thermal behaviour of different urban surface parameters (USPs) at large spatial scales is essential for strategic heat mitigation. 


Specific characteristics of the land cover impact the amount of diurnal heat it will absorb and emit into the atmosphere at nights.  contributing to  Urban Heat Island (UHI), 
Dark surface, higher heat storage capacity and large thermal inertia of concrete material contribute to a large solar radiation which will be stored in day time and emitted into the atmosphere at night [2,3].
This heat release has a significant impact on the thermal climate. The high air temperature of city centres is termed as the urban heat island (UHI) effect as compared to the sub-urban rural areas [4]."


The design process, however, fails to apply comprehensive life cycle environmental data to identify suitable construction solutions and urban management strategies that contribute to minimizing environmental impacts.
\cite{gao2019enhanced} The urban expansion with conversion of natural/vegetated cover to artificial surfaces has been broadly recognized as the main contributor to greater UHI effect in most cities (Imhoff et al 2010, Zhou et al 2015, Hu et al 2017, Liet al 2017).

The effects of urban structures and heavy usage of building materials (e.g. concretes and asphalts) on the land surface radiation budget and energy balance, which reduce the latent heat flux and increase the sensible heat flux (Oke 1982, Arnfield 2003). 

the heat released to the air from the urban surface was the major contributor to the increased temperature at nighttime. 


the contribution of urban surface parameters (USPs) for urban heating. 
The importance of city-scale implementation of USPs change to achieve maximum effectiveness in heat reduction \cite{Herath2021, agathangelidis2020urban}

The selection of pavement type requires an understanding of a local context of an area and characteristics of the pavements. 

urban surface parameters (USPs) for urban heating. 

notchanged yet: Increase in urban population across the globe has resulted in drastic rise in anthropogenic activities and urban surface modifications. These contribute to the hike of urban temperature above the temperature of surrounding rural areas. When this happens, the city is said to experience Urban Heat Island (UHI)~\citep{nwakaire2020urban}.




%



\subsection{Computer vision and semantic segmentation}

% Computer vision techniques have been widely applied to street-level imagery to map openness in cities~\citep{li2017building}, assess street-level urban greenery \citep{li2015assessing, ye2019measuring}, extract land use information from the built environment \citep{li2017building}, measure the visual quality of street space \citep{tang2019measuring}, visual enclosure~\citep{yin2016measuring} and sky exposure \citep{carrasco2015using}, and to detect traffic signs \citep{balali2015detection,campbell2019detecting}, urban landmarks \citep{lander2017inferring}, pavement defects \citep{Ma-etal-BMVC17,nolte2018assessment,7533052, jenkins2018deep, cao2020review}, and curb ramps \citep{hara2014tohme}. 
%
Emerging work has explored surface material classification via patch-level sampling and classification \citep{ferreira2017convolutional, ran2019rock} or with cameras directed at the surface~\citep{jain2018recognizing, xue2020differential}. In contrast, our work focuses on readily available street-level urban images \emph{in the wild} such that the paving material is only part of the overall scene. Pavement material classification has been used in safety and route-finding applications to alert pedestrians of upcoming obstacles~\citep{sun2019wide, sun2019deep,theodosiou2020first,kang2020safexr} and to help the visually impaired in identifying street entrances based on the change in surface materials captured by cellphones~\citep{jain2018recognizing}. 

Image classification and object detection have been frequently used in urban analysis~\citep{law2018street, nolte2018assessment, campbell2019detecting, miranda2020mosaic, kharazi2021flood}. However, semantic segmentation, which provides pixel-level predictions for object classes, has remained relatively under-utilized. 
%
Urban segmentation works~\citep{zhou2021using, kim2021decoding, zhang2018representing, wang2019perceptions} forego retraining or fine-tuning their models on their target datasets and rather rely only on publicly-available models which were pre-trained on datasets such as CityScapes~\citep{cordts2016cityscapes}, Mapillary~\citep{neuhold2017mapillary}, and ADE20K~\citep{zhou2017scene}. This reliance on pre-trained models not specific to the desired task limits analysis to the pre-defined object-classes included in those datasets~\citep{ahn2018learning}. Further, pre-trained models not fine-tuned on domain-specific data can yield sub-optimal performance~\citep{azizi2021big}.

We also contextualize our work concerning the developments in urban scene parsing and segmentation. Recent interest in autonomous vehicles has created significant demand for algorithms that can accurately incorporate high and low-level information from urban scenes, leading to notable segmentation improvements.
%
% To achieve this goal, various different models have been developed each trying to propose efficient techniques for learning representations of the images that helps extracting useful information from input image to make better final prediction \citep{bengio2013representation}. The challenge often lies in making use of both low and high-resolution representations \cite{}. 
%
Early work~\citep{zhao2017pyramid} incorporated multi-resolution processing into segmentation architectures to improve performance over a static-resolution approach. This has been followed by rapid developments in multi-scale pyramid-style networks including~\citep{he2019dynamic,ding2018context,he2019adaptive}. In particular, HRNet~\citep{sun2019high,wang2020deep} connects high-to-low resolution convolutions via parallel and repeated multi-scale fusions to better preserve low-resolution representations alongside the high-resolution ones in comparison to previous works such as~\cite{newell2016stacked,chen2018cascaded,yu2018deep}. A variant of HRNet, HRNet-W48, has shown superior performance across segmentation benchmarks such as Cityscapes and Mapillary Vista~\citep{sun2019deep} and is used as a key component of our segmentation framework. 

Attention-based mechanisms have been adopted in multiple semantic segmentation architectures \citep{huang2017semantic, fu2019dual, chen2016attention, li2018pyramid}. Instead of feeding multiple resized images into a shared network and merging the features to make the prediction, which can lead to sub-optimal results, the attention mechanism learns to assign different weights to multi-scale features at a pixel-level and uses the weighted sum of score-maps across all scales for the final prediction \citep{chen2016attention}. \citet{huang2017semantic} proposed RAN, a reversed attention mechanism that trains the model on the features which are not associated with the target class. The~network has three branches that simultaneously perform direct, reverse, and reversed-attention learning. Hierarchical multi-scale attention ~\citep{tao2020hierarchical}, proposes a model which learns to assign a relative weighting between adjacent scales. This method has shown to be four times more memory efficient and allows for larger crop sizes that can lead to more accurate results. 

We note that recent progress in self-supervised learning~\citep{chen2020big,he2020momentum,grill2020bootstrap} has lead to dramatic gains in image classification with limited annotated data alongside large collections of unlabeled images. As the architectures and training strategies for self-supervised classification depart significantly from those used for supervised urban image segmentation, we instead use active learning to address limited data concerns in order to make use of high-performing urban segmentation frameworks.

% In semantic segmentation models, the accuracy can vary on different scales \citep{tao2020hierarchical}. Lower inference resolution would better capture the global context, while higher inference resolutions would better deal with edges of objects/thin structures. The direct idea is to pass all different image scales through the neural network and then combine the output results by averaging or max pooling. However, combining the best predictions with poorer ones in this way will lead to sub-optimal results. To solve this problem, we apply the attention mechanism for combining multi-scale predictions at a pixel level.

\subsubsection{Active learning}

Deep network training requires a large number of annotated images to achieve generalization. In particular, semantic segmentation has the highest associated annotation cost as every pixel needs identification~\citep{pathak2015constrained} and modern cameras ubiquitously capture millions of pixels. The substantial cost of accurate annotation restricts the practicality of semantic segmentation on new datasets and tasks relevant to urban analysis~\citep{xie2020deal, montoya2014mind}. 

Active learning aims to achieve high accuracy with minimal labeled data by incorporating human supervision during training. By annotating images that the model struggles on or the most informative samples, fewer labeled instances are required to achieve similar performance when compared to supervised approaches where every image is densely annotated~\citep{settles2009active}. Common methods to active learning for vision usually follow a uncertainty-based~\citep{wang2016cost, gal2017deep} or a representation-based \citep{sener2017active, gissin2019discriminative} approach.
%
Active learning for semantic segmentation requires measurements of unlabeled image informativeness for segmentation networks~\citep{xie2020deal} and includes methods that use the entire image for sampling \citep{yang2017suggestive, kuo2018cost} and region-level methods which only require informative regions to query unlabeled data~\citep{mackowiak2018cereals, casanova2020reinforced}. We refer the reader to \citet{settles2009active} for an extensive review of active learning techniques.

% As inter-disciplinary research has examined how the built environment can influence health~\citep{lee2009design, NICKELSON2013179}, safety~\citep{ASADISHEKARI20151, AGHAABBASI2018475, naik2014streetscore, doi:10.1177/0042098008093386}, social inclusion, and social capital~\citep{toker2015walking}, objective measurement of the qualitative built environment features has become of key interest. 


% In the context of semantic segmentation of urban scenes, various papers proposed active learning techniques aiming at reducing annotation costs. \citet{kasarla2019region} proposed a region-based active learning method that makes use of super-pixels by only annotating 10\% of the pixels. The study leverages existing annotated urban dataset~\citep{cordts2016cityscapes} to run the experiments.  

% But AL is fairly new and less explored In the urban analysis context, . 

% \cite{golestaneh2020importance, kasarla2019region}


%We employed active learning to decrease the labeling cost by choosing the most informative sample to be annotated~\citep{gao2020consistency}. 

% and increase the variance of our data to have a more generalizable model~\citep{tao2020hierarchical}.


% methods such as  and Entropy \citep{shannon1948mathematical}, 

%

% The baseline network is the HRNet \citep{sun2019high,wang2020deep}



% This paper, enriches the existing measures of sidewalk assessment through developing a semantic segmentation model for a large scale classification of eight classes of paving materials, with a prominent accuracy. 

% sidewalk condition and presence of obstructions have been identified in
% national accessibility guidelines and recent pedestrian research as significant for pedestrian safety, mobility and quality of life.


% \cite{jain2018recognizing} Differentiating materials is harder than recognizing objects, even for the human eyes. Objects have well-defined shapes and high level attributes that can be quantified to identify them against a background, even in extreme lighting and weather conditions [19], [20]. On the other hand, texture attributes used for material recognition are a quantitative measure of the local and global arrange- ment of individual pixels.



% We employ semantic segmentation method to classify different materials of sidewalks and roads from street-level images. The multi-scale and pyramid network (MSPN) were most popular network for semantic segmentation recently. 




%The key advantage of HRNet-W48 is the multi-scale fusions which maintains high-resolution representations quite well. 




% All of these works are trying to find efficient methods to make use of the features from multiple levels through giving different priorities to different scales.



% % This way is much better than the simple aggregation way and can achieve fewer information losses in low-resolution representations. This information is critical for texture segmentation.








% \subsection{Street-view images to empower auditing}   


% Recently, street view images have gained popularity as a virtual audit tool \citep{rundle2011using, kelly2013using} since they can significantly reduce costs and time, expand the geographical area of the study \citep{badland2010can, charreire2014using, rzotkiewicz2018systematic}. The agreement level between the data collected through in-field and virtual audits have been tested in a number of studies. Majority of the reviewed studies showed a very high agreement between the results obtained using the two methods \citep{badland2010can, rundle2011using, phillips2017online, shatu2018development}. 

% Following legal actions taken by ADA, various cities such as NYC, Philadelphia, Seattle, and Portland ~\citep{lawsuit, multiplelawsuits}, sidewalks' assessment and repair have become the top priority for many cities. For instance, NYC needs to assess the condition and quality of all the city's 162,000 curbs to make sure they comply with the ADA requirements. Conventional methods of in-field audits fail to fulfill the task in timely manner without overwhelming costs. To put it in perspective, the city rained and employed 40 auditors in 2014 to audit the sidewalks and curb ramps but less than 1\% of curbs were assessed. This motivated several studies to come up with semi-automated or fully automated solutions. In Project sidewalk, \citet{saha2019project} designed a web-based tool to virtually identify accessibility problems at street segment level, by exploring the study area through GSV Images. Using the predefined labels, crowdworkers would virtually explore the designated region and annotate the problematic areas. 


==> old/results.tex <==


\section{Results}
In this section, we present the results of applying our trained model on held-out test sets. We do not rely on pixel-level accuracy to evaluate our model since sidewalks comprise a relatively small portion of each image, while road and background can occupy more than 70\% of most images, resulting in a significant class imbalance. This class imbalance creates an arbitrary high pixel-level accuracy, which is not a fair representation of the model's performance. 

\begin{figure*}
\centering
\includegraphics[width=0.8\linewidth]{figs/results_compressed.pdf}
\caption{Predictions of the model on the held-out test set. Fine details and boundaries of objects like poles, plants, wooden sticks, and fire hydrants are very precisely predicted. The model also segmented curb cuts (line 1 - column 2), different instances of the same material (3-1), (3-3), and visually similar materials of different classes (1-4). 
}
\label{fig:results}
\end{figure*}


\subsection{General evaluation metrics}
Table~\ref{tab:Results} presents class-level evaluation metrics, the mean Jaccard index (IoU), precision, and recall for our final model, which outputs ten classes in total, seven classes of sidewalk pavings, one extra class of street pavings - cobblestone - plus road and background. Excluding road and background, the model achieved 88.37\% accuracy, with hexagonal asphalt pavers and asphalt sidewalks having the highest accuracy measures. Overall, half of the pavement classes have IoU above 90\%. Concrete, the most prevalent and versatile material, can be classified with 88.7 accuracy, a robust result considering the high within-class variation (i.e., it comes in a variety of colors and textures). 
%
Granite/bluestone and granite block have the lowest accuracy (81.09 and 82.92 respectively), which can be partially explained by their visual similarity to dark concrete (or wet concrete), potentially leading to more false positive predictions.



\begin{table}[h!]
\centering
\caption{Evaluation metrics on the held-out test set}
\label{tab:Results}
\begin{tabular}{c|c|c|c}
% \cline{2-4}
%  & \multicolumn{3}{|c}{MaterialNet} \\ \hline
\hline
Label & IoU & Precision & Recall \\ \hline
Concrete & 88.69 & 0.95 & 0.93 \\
Brick & 91.79 & 0.95 & 0.96 \\
Granite/Bluestone & 81.09 & 0.85 & 0.95 \\
Asphalt & 92.58 & 0.96 & 0.97 \\
Mixed & 86.11 & 0.93 & 0.93 \\
Granite Block/Stone & 82.92 & 0.94 & 0.88 \\
Hexagonal Asphalt Paver & 92.81 & 0.98 & 0.95 \\
Cobblestone & 90.95 & 0.94 & 0.96 \\
Road & 99.01 & 0.99 & 1  \\
Background & 99.16 & 1 & 1 \\ \hline
\textbf{mIoU} & \multicolumn{3}{c}{90.51} \\ \hline
\textbf{mIoU (eight main classes)} & \multicolumn{3}{c}{88.37} \\ \hline
\end{tabular}
\end{table}

Fig.~\ref{fig:results} highlights some important cases, especially considering the \emph{in the wild} nature of GSV images. We can notice that CitySurfaces performs well in detecting boundaries between fine objects, like poles and plants, even in shadowed scenes (line 1 - column 1, 1-3, 2-1).
%
One interesting aspect of CitySurfaces is the ability to detect curb ramps in most scenes, even though it was not designed with such a goal. (1-1 and 2-2). 
%
Fig.~\ref{fig:results}(1-2) shows an area with patches of different materials and how the model can accurately classify each type. 
%
We can see that the model performs well in distinguishing between visually similar materials (3-2, 1-4), as well as visually different types of the same material (3-1).

% \newcolumntype{Z}{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}X}



\subsection{Evaluating the generalization capabilities of CitySurfaces}


As previously mentioned, we highlight that CitySurfaces was only trained using images from Boston and Manhattan. To demonstrate the generalization capabilities of CitySurfaces, we selected Chicago, Washington DC, Philadelphia, and Brooklyn (NYC's borough), to test the performance of our approach on different cities. 
%
To this end, for each city, we randomly sampled 200 street segments and obtained the street-view images at every five meters of each segment, from the left and right sides of the sidewalks. After data cleaning and pre-processing, we were left with roughly 600 images per city; these images were annotated using the model in block (b) then \emph{manually} checked and refined to create the test set. Table~\ref{tab:cityresults} illustrates the results of applying CitySurfaces on the test sets, both using a mIoU and a mean per-segment accuracy. This last measure was defined as a simple and more practical metric that measures whether the model could correctly detect the main dominant material in each street segment.
%
All tested cities had an accuracy greater than 82\%, with Brooklyn performing best, as expected since the borough's paving materials follow the same street design regulation as Manhattan.

\begin{table}[h!]
\centering
\caption{Segmentation results on the test sets of selected cities.}
\label{tab:cityresults}
\begin{tabular}{l|l|c}
\hline
City & \multicolumn{1}{c|}{mIoU} & Mean Per-Segment Accuracy \\ \hline
Brooklyn & 86.12 & 87.09 \\
Chicago & 84.31 & 86.52 \\
% Jersey City & 82.74 & 84.02 \\
Washington DC & 82.61 & 84.27 \\
Philadelphia & 82.81 & 83.46 \\
\hline
\end{tabular}
\end{table}

One of the major advantages of CitySurfaces is the ability to generate city-wide sidewalk material datasets, as can be seen in Fig.~\ref{fig:results}. This allows us to compare the distribution of different paving materials throughout cities, as depicted in Fig.~\ref{fig:radardiagram}.
%
As can be seen, concrete is the dominant material in all of the selected cities. Chicago has the highest number of asphalt sidewalks among the selected cities; Boston, Washington DC, and Philadelphia have a similar number of asphalt sidewalks, which come second to Chicago. Asphalt sidewalks are mainly used in suburban neighborhoods; that is why dense urban areas like Manhattan and Brooklyn have the lowest number of sidewalks paved with asphalt. Another interesting observation is the higher usage of granite / bluestone in Manhattan compared to Brooklyn, two boroughs of the same city. Granite is considered an expensive and decorative material, used mainly in commercial streets or historic neighborhoods, which signals the higher land value and income level of Manhattan, since maintenance and installation of decorative pavings are the owner's responsibility. 
%
Another interesting aspect is that Manhattan and Washington DC use more diverse and balanced material types.

\begin{figure}[t!]
\centering
\includegraphics[width=0.5\textwidth]{figs/materials_overview.pdf}
\caption{Comparison of the distribution of detected materials in six different cities. The star plots show the log of the number of sidewalk segments identified as having a given material.}
\label{fig:radardiagram}
\end{figure}



==> old/review_response.tex <==

Before responding to particular points raised, we would like to thank each of the reviewers for their carefully considered and constructive feedback regarding the research we present in this paper.  We particularly appreciate that all reviewers recognize its real-world utility and innovation and provided us with the opportunity to improve, strengthen, and resubmit our work after minor revision. We also acknowledge reviewers' reservations and are grateful for the helpful suggestions they make with regards to the paper’s limitations and for possible areas of improvement. We hope to significantly ease these reservations, and provide reassurances regarding the strength of our contribution to urban sustainability research.

We addressed all the comments made by the reviewers and included all the changes in a \emph{.tex} file, called \emph{CitySurfaces_revision.text}. In that file, all new entries are highlighted in blue and the removed texts from the original submission are highlighted in red with strike-through formatting. We will go through all the comments and will specify the changes together with their corresponding page and line number. 

First, we would like to address the comment regarding the relationship between surface materials and UHI (R2). Following the reviewers recommendation and to make the connection more clear, we added 12 extra references as well as a paragraph on page 2, lines 5-13, explaining how surface material can impact the UHI. We have made an attempt to extend this comment to the two other major areas impacted by the sidewalk pavements which was touched upon in the introduction, runoff water and accessibility. For each topic, one short paragraph was added. page 2, lines 13-17 (water runoff), lines 18-23 (accessibility).     

About the citation introducing UHI, as requested by R2, we removed the more recent paper (Mohajerani et al., 2017) and only kept the main one (Oke, 1982) in that sentence. The changes are highlighted on page 2, line 6. 

Regarding the concern raised by R2 about the long figure captions, we did our best in shortening the captions of the mentioned figures (1, 4, 11) as well as figure 2 (page 4) and 12 (page 14). Since some figures like fig. 4 (page 6) and 11 (page 13) are more complicated, the captions could not become significantly shorter but we kept only the necessary descriptions. 

In response to the great question raised by R2, asking whether our framework distinguishes materials of different classes based on their albedo value (or the visual charismatics such as brightness of color or reflectiveness, or it can be extended to do that, we have added a paragraph to the conclusion section, page 15 lines 26-35 to address this question. In short, our framework can be extended to classify materials based on such considerations, and in our future work, we plan to generate such dataset and combine it with shadow accumulation data to measure the city-scale UHI. 


Following the R3 recommendation, we have removed the first paragraph of the introduction and re-arranged the whole introduction section into a more sound and structured part. The first three pages of the article have been re-written and re-arranged to satisfy the raised concern. 

We would also like to thank R3 for the encouraging words regarding the possible impacts of our study on various urban policies and planning. We plan to make the model and all datasets created in this study publicly available through a GitHub repository. The link and name of the repository was removed to satisfy the double blind review requirements. 

Finally, we would like to thank each of the reviewers once again. We also hope that we have been able to satisfy the concerns each reviewer has raised and provided reassurances that we will be able to provide a camera-ready paper that reports our research effectively to the journal's audience. 








==> old/reviewes.tex <==
Reviewer #2: The authors present a study in which they propose the CitySurfaces framework. This framework uses an active learning strategy and combines it computer vision techniques for localization categorization of sidewalk pavement materials based on street images (e.g. from Google street view). The paper is well-written and structured. 

The authors attempt to relate to the issue of UHIs, however, some additional text would be needed to fully justify this link in my opinion. 


I only have a couple of other small comments.

"phenomenon called Urban Heat Island (UHI) effect (Mohajerani et al., 2017; Oke, 1982); please put first publications first. The paper by Mohajerani from 2017 will certainly not have introduced the concept of UHI, so I would omit this one, or at least place "e.g." in front of the references.

Some figure captions (Fig. 1,4,11) are very long. Please shorten them by excluding less relevant text.

Section 3.1: a distinction between materials is made. 
For UHI studies not only the type of material (and related thermal properties as specific heat capacity, density, thermal conductivity) is of importance, but also albedo values. 
white concrete pavement will have other effects on the thermal conditions as an almost black pavement of the same material. 
Does the framework consider these differences? Can the framework be extended to include this as well? Please elaborate on this aspect.

TODO: EXPLAIN about ALBEDO and that our model cannot directly measure this but since it is trained on detecting the standard materials mentioned in the city guides, it can be used to calculate albedo given that we know the value for those materials. 
Also, it is a framework and it can be extended as we showed, to detect many other materials,



Reviewer #3: The paper proposes a machine learning method to detect sidewalks surfaces using semantic segmentation on street view images available online. The authors develop a very rigorous methodology, which is specially challenging in their case, since sidewalks seldom occupy more than 30\% of the visual information in street view images, are often obstructed by vehicles and other elements deployed on sidewalks (trees, benches, etc.), and their reduced area are particularly affected by sunlight conditions. The authors propose a multi-step approach to address these challenges, and they do it very well and in a detailed manner. Besides the technical quality, the paper addresses an important topic: assessment of sidewalk materials. What is also noteworthy is the transferability of the method, tested in other cities for which there is no ground truth.

I have one minor, but essential, suggestion: the first paragraph of the paper (from "The process of urbanization..." to "... uninformed decisions of the past" is not only totally irrelevant for the paper, but it also is shallow in comparison with the remaining of the paper, and diverts the reader's attention from the main focus.

I wonder if the authors will make the model available on Github, which could be extremely valuable for other scholars to test it in other cities, as well as for public officials to define policies and additional studies—for instance, level of physical activity in different areas of the city in relation to pavement, type of pavement and socioeconomic profile of neighborhoods, pedestrian accidents and type of pavement, etc.
   



